Team Northeastern's Approach to ANA XPRIZE Avatar Final Testing: A Holistic Approach to Telepresence and Lessons Learned

This paper reports on Team Northeastern's Avatar system for telepresence, and our holistic approach to meet the ANA Avatar XPRIZE Final testing task requirements. The system features a dual-arm configuration with hydraulically actuated glove-gripper pair for haptic force feedback. Our proposed Avatar system was evaluated in the ANA Avatar XPRIZE Finals and completed all 10 tasks, scored 14.5 points out of 15.0, and received the 3rd Place Award. We provide the details of improvements over our first generation Avatar, covering manipulation, perception, locomotion, power, network, and controller design. We also extensively discuss the major lessons learned during our participation in the competition.

==> tables/power_budget.tex <==
\begin{table}[h]
\centering
\caption{Remote System Power Budget: Lists major power sinks and nominal power consumption. When operating untethered, $\sim$1kWh is provided by two Valence U1-12RJ batteries, allowing approximately 2-3 hours of operation based on empirical testing. Note that estimates are slightly pessimistic to reflect variations in real world usage.}
    \label{tab:power_budget}
    \begin{tabular*}{\columnwidth}{| m{5em} | m{1.5cm} | m{4.42cm} |}
        \hline
         System & Nominal Power Draw & Notes \\
         \hline\hline
         Panda Arms & 2$\times$125W & Mean Well TS-1000 provides  AC power.\\ 
         \hline
         Computers & 2$\times$60-120W & We used 2 gaming NUC's \\
         \hline 
         Vector Base & 100W & Not Measured Precisely. Most of the time it is stationary.\\
         \hline
         Haptic Grippers & 20-80W & Power draw is low when not using the grippers\\
         \hline
         Other Systems & $<30$W & Includes Cameras, lasers, fans, emergency stop circuitry\\
         \hline\hline
         Total & $\sim500$W & Implies an operating time of approximately 2 hours.\\
         \hline
    \end{tabular*}
    
\end{table}

